Can Pretrained Language Models Derive Correct Semantics from Corrupt Subwords under Noise?

For Pretrained Language Models (PLMs), their susceptibility to noise has recently been linked to subword segmentation. However, it is unclear which aspects of segmentation affect their understanding. This study assesses the robustness of PLMs against various disrupted segmentation caused by noise. An evaluation framework for subword segmentation, named Contrastive Lexical Semantic (CoLeS) probe, is proposed. It provides a systematic categorization of segmentation corruption under noise and evaluation protocols by generating contrastive datasets with canonical-noisy word pairs. Experimental results indicate that PLMs are unable to accurately compute word meanings if the noise introduces completely different subwords, small subword fragments, or a large number of additional subwords, particularly when they are inserted within other subwords.

==> delete-vowel-repetition.tex <==
spurious segmentation \footnote{It is spurious because the compositionality of the subwords for misspelled words is different from those during the training phrase}.

a) complete corruption: can PLMs restore word meanings from completely different subwords? 
b) partial corruption: if not, can PLMs restore word meanings from partial subwords?
b) additive corruption: can PLMs still infer word meanings with the insertion of irrelevant subwords? 


However, subword representations may not encode character information. Even though it has such character information, PLMs are not pretrained with an explicit objective to generate similar representations for similar compositionality of characters. 

\textit{vowel-repetition}: We repeat the first vowel letter to exaggerate a stronger emotion (e.g., "taasty"). They may provide nuances of semantic information compared to the formalized word forms and would be meaningful for tasks like sentiment analysis and identifying the reading level of documents.


